SCATTER: Selective Context Attentional Scene Text Recognizer

Scene Text Recognition (STR), the task of recognizing text against complex image backgrounds, is an active area of research. Current state-of-the-art (SOTA) methods still struggle to recognize text written in arbitrary shapes. In this paper, we introduce a novel architecture for STR, named Selective Context ATtentional Text Recognizer (SCATTER). SCATTER utilizes a stacked block architecture with intermediate supervision during training, that paves the way to successfully train a deep BiLSTM encoder, thus improving the encoding of contextual dependencies. Decoding is done using a two-step 1D attention mechanism. The first attention step re-weights visual features from a CNN backbone together with contextual features computed by a BiLSTM layer. The second attention step, similar to previous papers, treats the features as a sequence and attends to the intra-sequence relationships. Experiments show that the proposed approach surpasses SOTA performance on irregular text recognition benchmarks by 3.7\% on average.

==> tables/ablation.tex <==
\begin{table*}
\small
\begin{center}
\bgroup
\def\arraystretch{1.1}
\centering
  \begin{center}
  \captionsetup[table]{skip=10pt}
    \caption{Ablation studies by changing model hyper-parameters.
    We refer to our re-trained model using the code of Baek et al. 2019 as Baseline.
    Using intermediate supervision helps to boost results and enables stacking more blocks. Increasing the number of blocks has positive impacts on the recognition performance. * Regular Text and Irregular Text columns are  weighted (by size) average results on the regular and irregular datasets respectively.}
    \label{tab:ablation}
    \footnotesize
    \begin{tabular}{|P{0.3cm}|P{1.2cm}|P{0.85cm}|P{1.0cm}|P{1.0cm}|P{0.7cm}|P{0.65cm}|P{0.5cm}P{0.3cm}P{0.3cm}P{0.5cm}|P{0.5cm}P{0.4cm}P{0.4cm}|P{0.85cm}|P{1.0cm}|} 
      \hline
      \multirow{2}{*}{{Sec}} & \multirow{2}{*}{{Method}} & {CTC} & {Attention} & {Selective} & {LSTM} & {N} & \multicolumn{4}{c|}{{Regular test dataset}} & \multicolumn{3}{c|}{{Irregular test dataset}} & {Regular} & {Irregular}\\
       & & {Decoder} & {Decoders} & {Decoders} & {Layers} & {Blocks} & IIIT5K & SVT & IC03 & IC13 & IC15 & SVTP & CUTE & {Text*} & {Text*}\\
      \hline
      & \cite{Baek2019clova} & 0 & 1 & - & 2 & - & 87.9 & 87.5 & 94.9 & 92.3  & 71.8 & 79.2  & 74.0 & \GreyHeatmap{89.8} & \GreyHeatmapB{73.7} \\ 
      \cline{2-16}
      & Baseline & 0  & 1 & - & 2 & - & 91.7 & 87.9 & 95.1 & 92.3  & 76.3 & 79.4  & 81.9 & \GreyHeatmap{91.9} & \GreyHeatmapB{77.5} \\
      \cline{2-16}
      \multicolumn{1}{|c|}{(a)} & Baseline & 1  & 1 & - & 2 & - & 91.9 & 87.5 & 95.2 & 93.4 & 77.7 & 80.1  & 84.8 & \GreyHeatmap{92.2}& \GreyHeatmapB{79.0} \\
      \cline{2-16}
      & \AlgoName & 0  & - & 1 & 2 & 1 & 92.3 & 88.6 & 95.5 & 93.1 & 79.1 & 81.6  & 82.6 & \GreyHeatmap{92.5} & \GreyHeatmapB{79.9} \\
      \cline{2-16}
      & \AlgoName & 1  & - & 1 & 2 & 1 & 92.2 & 91.7 & 95.0 & 92.3  & 79.5 & 84.5  & 84.7 & \GreyHeatmap{92.6} & \GreyHeatmapB{81.1}  \\
      \hline
      \hline
       & \AlgoName & 0  & - & 1 & 4 & 2 & 92.0 & 90.3 & 94.8 & 92.6 & 79.5 & 83.6  & 83.7 & \GreyHeatmap{92.3} & \GreyHeatmapB{80.8} \\
      \cline{2-16}
      \multicolumn{1}{|c|}{(b)} & \AlgoName & 0  & - & 2 & 4 & 2 &  92.2 & 89.5 & 95.5 & 93.5 & 79.9 & 83.1  & 85.4 & \GreyHeatmap{92.6} & \GreyHeatmapB{81.2} \\
      \cline{2-16}
      & \AlgoName & 1  & - & 1 & 4 & 2 & 92.9 & 89.0 & 95.5 & 93.4  & 80.9 & 83.4  & 81.6 & \GreyHeatmap{92.9} & \GreyHeatmapB{81.5} \\
      \cline{2-16}
      & \AlgoName & 1  & - & 2 & 4 & 2 & 92.4 & 90.9 & 96.5 & 93.1 &  80.5 & 84.8  & 86.1 & \GreyHeatmap{93.0} & \GreyHeatmapB{81.9} \\
      \hline
      \hline
      & \AlgoName & 1  & - & 3 & 6 & 3 & 92.6 & 90.4 & 95.6 & 92.9  & 80.8 & 84.9  & 87.2 & \GreyHeatmap{93.0} & \GreyHeatmapB{82.3} \\
      \cline{2-16}
      \multicolumn{1}{|c|}{(c)} & \AlgoName & 1  & - & 4 & 8 & 4 & 93.5 & 90.1 & 95.9 & 93.9 &  81.3 & 85.6  & 85.4 & \GreyHeatmap{93.6} & \GreyHeatmapB{82.6} \\
      \cline{2-16}
      & \AlgoName & 1  & - & 5 & 10 & 5 & 92.9 & 89.7 & 95.7 & 93.9 & 81.4 & 85.2  & 84.1 & \GreyHeatmap{93.2} & \GreyHeatmapB{82.4} \\
      \cline{2-16}
      & \AlgoName & 1  & - & 6 & 12 & 6 & 92.9 & 88.3 & 94.7 & 93.1 & 82.0 & 83.9  & 84.4 & \GreyHeatmap{92.7} & \GreyHeatmapB{82.6} \\
      \hline
    \end{tabular}
  \end{center}
\egroup
\end{center}
\end{table*}


==> tables/clova_full_evaluation.tex <==
\begin{table*}
\normalsize
\begin{center}
\bgroup
\def\arraystretch{1.1}
\centering
  \begin{center}
    \caption{Performance of out model and other State-Of-The-Art methods on public datasets. All values are reported as precentage (\%). “Cl ReIm” is Clova re-implemented \cite{Baek2019clova}. "None" means that no lexicon was used.}
    \label{tab:table0}
    \begin{tabular}{|P{2.0cm}|P{1cm}|P{0.75cm}|P{0.75cm}P{0.75cm}|P{0.75cm}P{0.75cm}|P{0.75cm}P{0.75cm}|P{1cm}|P{1cm}|} 
      \hline
      \multirow{2}{*}{\textbf{Method}} & \textbf{IIIT5K} & \textbf{SVT} & \multicolumn{2}{c}{\textbf{IC03}} & \multicolumn{2}{|c}{\textbf{IC13}} & \multicolumn{2}{|c|}{\textbf{IC15}} & \textbf{SVTP} & \textbf{CUTE}\\
      &  3000 & 647 & 860 & 867 & 857 & 1015 & 1881 & 2077 & 645 & 288\\
      \hline
      \AlgoName (1 Block) & 92.2 & 91.7 & 94.5 & 95.0 & - & 92.3 & - & 79.5 & 84.5 & 84.7\\
      \hline
      \AlgoName (2 Block) & 92.4 & 90.9 & - & 96.5 & - & 93.1 & - & 80.5 & 84.8 & 86.1\\
      \hline
      \AlgoName (3 Block) & 92.6 & 90.4 & - & 95.6 & - & 92.9 & - & 80.8 & 84.9 & 87.2\\
      \hline
      \AlgoName (4 Block) & 93.5 & 90.1 & - & 95.9 & - & 93.9 & - & 81.3 & 85.6 & 85.4\\
      \hline
      \AlgoName (5 Block) & 92.9 & 89.7 & - & 95.7 & - & 93.9 & - & 81.4 & 85.2 & 84.1\\
      \hline
      \AlgoName (6 Block) & 92.9 & 88.3 & - & 94.7 & - & 93.1 & - & 82.0 & 83.9 & 84.4\\
      \hline
    \end{tabular}
  \end{center}
\egroup
\end{center}
\end{table*}

==> tables/decoder_limit.tex <==
\begin{table}[t]
\normalsize
\begin{center}
\bgroup
\def\arraystretch{1.1}
\centering
  \begin{center}
  \captionsetup[table]{skip=10pt}
    \caption{Performance of each decoder and the oracle (the oracle performance is calculated post-process, that is given the ground truth).}
    \label{tab:decoder_limit}
    \footnotesize
    \begin{tabular}{|P{1.0cm}|P{0.70cm}P{0.50cm}P{0.50cm}P{0.50cm}|P{0.50cm}P{0.50cm}P{0.65cm}|} 
      \hline
      \textbf{Decoder} & \textbf{IIIT5K} & \textbf{SVT} & \textbf{IC03} & \textbf{IC13} & \textbf{IC15} & \textbf{SVTP} & \textbf{CUTE}\\
      \hline
      $CTC$ & 89.8 & 85.5 & 93.1 & 90.6 & 68.0 & 75.7 & 77.4\\
      \hline
      $Attn_1$ & 93.2 & 90.1 & 95.6 & 93.8 & \textbf{81.8} & 84.8 & 84.8\\
      \hline
      $Attn_2$ & \textbf{93.5} & 90.6 & 95.6 & 94.0 & 81.1 & 84.0 & \textbf{85.4}\\
      \hline
      $Attn_3$ & 93.4 & \textbf{90.9} & 95.8 & \textbf{94.3} & 81.3 & 83.9 & 84.4\\
      \hline
      Final & \textbf{93.5} & 90.1 & \textbf{95.9} & 93.9 & 81.3 &  \textbf{85.6} & \textbf{85.4}\\
      \hline
      \hline
      Oracle & 95.7 & 93.5 & 97.2 & 95.9 & 85.4 & 87.9 & 88.6\\
      \hline
    \end{tabular}
  \end{center}
\egroup
\end{center}
\end{table}


==> tables/different_decoders.tex <==
\begin{table}
\normalsize
\begin{center}
\bgroup
\def\arraystretch{1.1}
\centering
  \begin{center}
    \caption{Predictions made by the different decoders. “GT” stands for the ground-truth annotation.}
    \label{tab:different_heads}
    \begin{tabular}{|P{1.1cm}|P{1.3cm}P{1.3cm}|P{1.0cm}P{1.5cm}|} 
      \hline
      \multirow{2}{*}{\textbf{Decoder}} & \multicolumn{2}{c|}{\textbf{Regular Text}} & \multicolumn{2}{c|}{\textbf{Irregular Text}}\\
      & \includegraphics[width=1.6cm]{latex/figures/council.jpg} & \includegraphics[width=1.4cm]{latex/figures/copies.jpg} & \includegraphics[width=1.1cm, height=0.5cm]{latex/figures/BMW.jpg} & \includegraphics[width=1.5cm]{latex/figures/BRASSERIE.jpg}\\
      \hline
      $CTC$ & \textcolor{red}{o}ouncil & \textcolor{red}{g}op\textcolor{red}{t}es & bm\textcolor{red}{\_} & \textcolor{red}{u}rasserie\\
      \hline
      $Attn_1$ & council & cop\textcolor{red}{t}es & \textcolor{red}{on} & \textcolor{red}{d}rasserie\\
      \hline
      $Attn_2$ & council & copies & bmw & \textcolor{red}{\_}rasserie\\
      \hline
      $Attn_3$ & council & copies & \textcolor{red}{any} & \textcolor{red}{\_}rasserie\\
      \hline
      Final & council & copies & bmw & brasserie\\
      \hline
      \hline
      GT & council & copies & bmw & brasserie\\
      \hline
    \end{tabular}
  \end{center}
\egroup
\end{center}
\end{table}

==> tables/handwrite_results.tex <==
\begin{table}[ht]
\begin{center}
\small
\caption{Results on three handwriting benchmarks datasets. Results show that SCATTER bla bla We refer to our re-trained model using the code of Baek et al. 2019 as Baseline. }
\label{tab:lstm}
\footnotesize
\bgroup
\def\arraystretch{1.1}
    \begin{tabular}{|P{1.5cm}|P{1.5cm}|P{1.0cm}|P{1.0cm}|P{1.0cm}|} 
      \hline
      \textbf{Method} & \textbf{\# Blocks} & \textbf{IAM} & \textbf{CVL}  & \textbf{RIMES}\\
      \hline
      Baseline & - & 75.7 & 77.1 & 87.7 \\
      \hline
      SCATTER & 1 & 76.2 & 76.2 & - \\
      \hline
      SCATTER & 2 & 77.1 & 76.6 & - \\
      \hline
      SCATTER & 3 & 77.4 & 76.4 & - \\
      \hline
      SCATTER & 4 & 78.1 & 77.0 & - \\
      \hline
    \end{tabular}
\egroup
\end{center}
\end{table}

==> tables/infer_time.tex <==
\begin{table}[ht]
\begin{center}
\small
\caption{The effect of the number of LSTM layers on inference time.}
\label{tab:infer_time}
\footnotesize
\bgroup
\def\arraystretch{1.1}
    \begin{tabular}{|P{1.1cm}|P{1.7cm}|P{1.5cm}|P{1.4cm}|} 
      \hline
      \textbf{N Blocks} & \textbf{LSTM Layers} & \textbf{Inference Time (ms)} & \textbf{Training Params} x$10^6$ & \textbf{Inference Params} x$10^6$\\
      \hline
      Standard & 2 & 27.6 & 49.6 & 49.6 \\
      \hline
      1 & 2 & 35.3 & 60.4 & -\\
      \hline
      2 & 4 & 38.5 & 74.9 & -\\
      \hline
      3 & 6 & 41.2 & 89.4 & -\\
      \hline
      4 & 8 & 49.1 & 103.9 & -\\
      \hline
      5 & 10 & 51.5 & 118.4 & - \\
      \hline
      6 & 12 & 54.1 & 132.9 & -\\
      \hline
    \end{tabular}
\egroup
\end{center}
\end{table}

==> tables/infere_time_rebutal.tex <==
\begin{table}[ht]
\begin{center}
\scriptsize
\caption{The effect of stacking block on computational cost. We refer to our re-trained model using the code of Baek et al. 2019 as Baseline. }
\label{tab:infere_time}
\scriptsize
\bgroup
\def\arraystretch{1.1}
    \begin{tabular}{|c|c|c|c|c|} 
      \hline
      \textbf{\# Blocks} & \textbf{LSTM Layers} & \textbf{Regular Text} & \textbf{Irregular Text} & \textbf{Time (ms)}\\
      \hline
      Beak et al. & 2 & 89.8 & 73.7 & 27.6 \\
      \hline
      Baseline & 2 & 91.9 & 77.5 & 37.2 \\
      \hline
      \hline
      1 & 2 & 92.6 & 81.1 & 39.4 \\
      \hline
      2 & 4 & 93.0 & 81.9 & 41.9 \\
      \hline
      3 & 6 & 93.0 & 82.3 & 44.6 \\
      \hline
      4 & 8 & 93.6 & 82.6 & 47.3 \\
      \hline
    \end{tabular}
\egroup
\end{center}
\end{table}

==> tables/lstm.tex <==
\begin{table}[ht]
\begin{center}
\small
\caption{The effect of the number of BiLSTM layers used on recognition accuracy. Only by using SCATTER we are able to add BiLSTM layer to improve results. Regular Text and Irregular Text columns are weighted (by size) average results on the regular and irregular datasets.
We refer to our re-trained model using the code of Baek et al. 2019 as Baseline. }
\label{tab:lstm}
\footnotesize
\bgroup
\def\arraystretch{1.1}
    \begin{tabular}{|P{1.3cm}|P{1.7cm}|P{1.6cm}|P{1.8cm}|} 
      \hline
      \textbf{\# Blocks} & \textbf{LSTM Layers} & \textbf{Regular Text} & \textbf{Irregular Text}\\
      \hline
      Baseline & 1 & 91.6 & 76.6 \\
      \hline
      Baseline & 2 & 91.9 & 77.5 \\
      \hline
      Baseline & 3 & 91.2 & 76.4 \\
      \hline
      Baseline & 4 & 91.0 & 75.6 \\
      \hline
      \hline
      1 & 2 & 92.6 & 81.1 \\
      \hline
      2 & 4 & 93.0 & 81.9 \\
      \hline
      3 & 6 & 93.0 & 82.3 \\
      \hline
      4 & 8 & 93.6 & 82.6 \\
      \hline
      5 & 10 & 93.2 & 82.3 \\
      \hline
      6 & 12 & 92.7 & 82.6 \\
      \hline
    \end{tabular}
\egroup
\end{center}
\end{table}



% \begin{table}[ht]
% \begin{center}
% \small
% \caption{The effect of the number of BiLSTM layers in each block on recognition accuracy. Only by using SCATTER we are able to add BiLSTM layer to improve results. Regular Text and Irregular Text columns are weighted (by size) average results on the regular and irregular datasets.
% We refer to our re-trained model using the code of Baek et al. 2019 Baseline. }
% \label{tab:lstm}
% \footnotesize
% \bgroup
% \def\arraystretch{1.1}
%     \begin{tabular}{|P{1.3cm}|P{1.7cm}|P{1.6cm}|P{1.8cm}|} 
%       \hline
%       \textbf{\# Blocks} & \textbf{LSTM Layers} & \textbf{Regular Text} & \textbf{Irregular Text}\\
%       \hline
%       Baseline & 1 & 91.6 & 76.6 \\
%       \hline
%       Baseline & 2 & 91.9 & 77.5 \\
%       \hline
%       Baseline & 3 & 91.2 & 76.4 \\
%       \hline
%       Baseline & 4 & 91.0 & 75.6 \\
%       \hline
%       \hline
%       1 & 1 & 92.8 & 80.8 \\
%       \hline
%       1 & 2 & 92.6 & 81.1 \\
%       \hline
%       1 & 3 & 92.8 & 81.9 \\
%       \hline
%       1 & 4 & 93.3 & 81.8 \\
%       \hline
%       \hline
%       2 & 2 & 92.9 & 81.9 \\
%       \hline
%       2 & 4 & 93.0 & 81.9 \\
%       \hline
%       2 & 6 & 92.8 & 82.4 \\
%       \hline
%       2 & 8 & 92.9 & 82.1 \\
%       \hline
%       \hline
%       3 & 3 & 92.9 & 82.3 \\
%       \hline
%       3 & 6 & 93.0 & 82.3 \\
%       \hline
%       3 & 9 & 92.8 & 82.3 \\
%       \hline
%       3 & 12 & 92.7 & 81.5 \\
%       \hline
%       \hline
%       4 & 4 & 92.7 & 82.0 \\
%       \hline
%       4 & 8 & 93.6 & 82.6 \\
%       \hline
%       4 & 12 & 92.9 & 82.7 \\
%       \hline
%       4 & 16 & 93.1 & 82.0 \\
%       \hline
%     \end{tabular}
% \egroup
% \end{center}
% \end{table}

==> tables/prune.tex <==
\begin{table}[h]
\begin{center}
\small
\caption{Average test accuracy at intermediate decoding stages of the network, compared across different training network depths. * Regular Text and Irregular Text columns are weighted (by size) average results on the regular and irregular datasets respectively.}
\label{tab:prune}
\footnotesize
\bgroup
\def\arraystretch{1.1}
    \begin{tabular}{|P{1.0cm}|P{1.6cm}|P{1.6cm}|P{1.0cm}|P{1.0cm}|} 
      \hline
      \textbf{Training Blocks} & \textbf{N Blocks After Pruning} & \textbf{N LSTM Layers After Pruning} & \textbf{Regular Text*} & \textbf{Irregular Text*}\\
      \hline
      1 & 1 & 2 & 92.6 & 81.1 \\
      \hline
      \hline
      2 & 1 & 2 & 92.8 & 82.3 \\
      \hline
      2 & 2 & 4 & 93.0 & 81.9 \\
      \hline
      \hline
      3 & 1 & 2 & 92.5 & 82.1 \\
      \hline
      3 & 2 & 4 & 92.7 & 82.5 \\
      \hline
      3 & 3 & 6 & 93.0 & 82.3 \\
      \hline
      \hline
      4 & 1 & 2 & 93.3 & 82.7 \\
      \hline
      4 & 2 & 4 & 93.6 & 82.1 \\
      \hline
      4 & 3 & 6 & 93.7 & 82.2 \\
      \hline
      4 & 4 & 8 & 93.6 & 82.6 \\
      \hline
      \hline
      5 & 1 & 2 & 93.0 & 81.9 \\
      \hline
      5 & 2 & 4 & 93.1 & 82.8 \\
      \hline
      5 & 3 & 6 & 93.3 & 82.1 \\
      \hline
      5 & 4 & 8 & 93.1 & 82.3 \\
      \hline
      5 & 5 & 10 & 93.2 & 82.4 \\
      \hline
    \end{tabular}
\egroup
\end{center}
\end{table}

==> tables/sota_results.tex <==
\newcommand\dunderline[3][-1pt]{{%
  \setbox0=\hbox{#3}
  \ooalign{\copy0\cr\rule[\dimexpr#1-#2\relax]{\wd0}{#2}}}}
\begin{table*}
\small
\begin{center}
\bgroup
\def\arraystretch{1.1}
\centering
  \begin{center}
  \captionsetup[table]{skip=5pt}
    \caption{Scene text recognition accuracies (\%) over seven public benchmark test datasets (number of words in each dataset are shown below the title). No lexicon is used.  In each column, the best performing result is shown in \textbf{bold} font, and the second best result is shown with an \underline{underline}. Average columns are weighted (by size) average results on the regular and irregular datasets. "*" indicates using both word-level and character-level annotations for training. "\textdagger" indicates model trained with end-to-end detection and recognition.}
    \label{tab:sota_results}
    \footnotesize
    \begin{tabular}{|P{4.0cm}|P{1cm}P{0.75cm}P{0.75cm}P{0.75cm}|P{1.0cm}|P{0.75cm}P{1cm}P{1cm}|P{1.0cm}|} 
      \hline
      \multirow{3}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Regular test dataset}} & \multicolumn{4}{c|}{\textbf{Irregular test dataset}}\\
      & IIIT5K & SVT & IC03 & \multicolumn{1}{c}{IC13} & \textbf{Average} & IC15 & SVTP & \multicolumn{1}{c}{CUTE} & \textbf{Average}\\
      & 3000 & 647 & 867 & \multicolumn{1}{c}{1015} & 5529 & 2077 & 645 & \multicolumn{1}{c}{288} & 3010\\
      \hline
      CRNN (2015) \cite{Bai2015crnn} & 78.2 & 80.8 & 89.4 & 86.7 & 81.8 & - & - & -& - \\
      \hline
      ATR (2017) \cite{Xiao2017atn}* & - & - & - & - & - & - & 75.8 & 69.3 & -\\
      \hline
      FAN (2017) \cite{bai2017accurate}* & 87.4 & 85.9 & 94.2 & 93.3 & 89.4 & 70.6 & - & - & -\\
      \hline
      Char-Net (2018) \cite{Wei2018charnet}* & 83.6 & 84.4 & 91.5 & 90.8 & 86.2 & 60.0 & 73.5 & - & -\\
      \hline
      AON (2018) \cite{Zhanzhan2018aon} & 87.0 & 82.8 & 91.5 & - & - & 68.2 & 73.0 & 76.8 & 70.0\\
      \hline
      EP (2018) \cite{bai2018edit}* & 88.3 & 87.5 & 94.6 & 94.4 & 90.3 & 73.9 & - & - & -\\
      \hline
      SSFL (2018) \cite{Yang2018cano} & 89.4 & 87.1 & 94.7 & 94.0 & 90.8 & - & 73.9 & 62.5 & -\\
      \hline
      NRTR (2018) \cite{Bai2018aster} & 86.5 & 88.3 & 95.4 & \dunderline{0.7pt}{94.7} & 89.6 & - & - & - & -\\
      \hline
      Baek et al. (2019) \cite{Baek2019clova} & 87.9 & 87.5 & 94.9 & 92.3 & 89.8 & 71.8 & 79.2 & 74.0 & 73.6\\
      \hline
      ASTER (2019) \cite{Bai2018aster} & 93.4 & 89.5 & 94.5& 91.8 & 92.8 & 76.1 & 78.5 & 79.5 & 76.9\\
      \hline
      SAR (2019) \cite{Wang2019sar} & 91.5 & 84.5 & - & 91.0 & - & 69.2 & 76.4 & 83.3 & 72.1\\
      \hline
      ESIR (2019) \cite{Zhan2019esir} & 93.3 & 90.2 & - & 91.3 & - & 76.9 & 79.6 & 83.3 & 78.1\\
      \hline
      MORAN (2019) \cite{Luo2019moran} & 91.2 & 88.3 & 95.0 & 92.4 & 91.7 & 68.8 & 76.1 & 77.4 & 71.2\\
      \hline
      Mask TextSpotter (2019) \cite{liao2019mask}*\textdagger & \textbf{95.3} & \textbf{91.8} & 95.0 & \textbf{95.3} & \textbf{94.8} & 78.2 & 83.6 & \textbf{88.5} & 80.0\\
      \hline
      \hline
      \AlgoName (1 Block) & 92.2 & \dunderline{0.7pt}{91.7} & 95.0 & 92.3 & 92.6 & 79.5 & 84.5 & 84.7 & 81.1 \\
      \hline
      \AlgoName (2 Block)& 92.4 & 90.9 & \textbf{96.5} & 93.1 & 93.0 & 80.5 & 84.8 & 86.1 & 81.9\\
      \hline
      \AlgoName (3 Block) & 92.6 & 90.4 & 95.6 & 92.9 & 93.0 & \dunderline{0.7pt}{80.8} & \dunderline{0.7pt}{84.9} & \dunderline{0.7pt}{87.2} & \dunderline{0.7pt}{82.3}\\
      \hline
      \AlgoName (4 Block) & \dunderline{0.7pt}{93.5} & 90.1 & \dunderline{0.7pt}{95.9} & 93.9 & \dunderline{0.7pt}{93.6} &  \textbf{81.3} & \textbf{85.6} & 85.4 & \textbf{82.6}\\
      \hline
    \end{tabular}
  \end{center}
\egroup
\end{center}
\end{table*}

==> tables/sota_results_fix_short.tex <==
\newcommand\dunderline[3][-1pt]{{%
  \setbox0=\hbox{#3}
  \ooalign{\copy0\cr\rule[\dimexpr#1-#2\relax]{\wd0}{#2}}}}
\begin{table*}
\small
\begin{center}
\bgroup
\def\arraystretch{1.1}
\centering
  \begin{center}
  \captionsetup[table]{skip=5pt}
    \caption{Scene text recognition accuracies (\%) over seven public benchmark test datasets (number of words in each dataset are shown below the title). No lexicon is used.  In each column, the best performing result is shown in \textbf{bold} font, and the second best result is shown with an \underline{underline}. Average columns are weighted (by size) average results on the regular and irregular datasets. "*" indicates using both word-level and character-level annotations for training. "\textdagger" indicates model trained with end-to-end detection and recognition.}
    \label{tab:sota_results}
    \footnotesize
    \begin{tabular}{|P{4.0cm}|P{1cm}P{0.75cm}P{0.75cm}P{0.75cm}|P{1.0cm}|P{0.75cm}P{1cm}P{1cm}|P{1.0cm}|} 
      \hline
      \multirow{3}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Regular test dataset}} & \multicolumn{4}{c|}{\textbf{Irregular test dataset}}\\
      & IIIT5K & SVT & IC03 & \multicolumn{1}{c}{IC13} & \textbf{Average} & IC15 & SVTP & \multicolumn{1}{c}{CUTE} & \textbf{Average}\\
      & 3000 & 647 & 867 & \multicolumn{1}{c}{1015} & 5529 & 2077 & 645 & \multicolumn{1}{c}{288} & 3010\\
      \hline
      Baek et al. (2019)  & 87.9 & 87.5 & 94.9 & 92.3 & 89.8 & 71.8 & 79.2 & 74.0 & 73.6\\
      \hline
      ASTER (2019)  & 93.4 & 89.5 & 94.5& 91.8 & 92.8 & 76.1 & 78.5 & 79.5 & 76.9\\
      \hline
      SAR (2019)  & 91.5 & 84.5 & - & 91.0 & - & 69.2 & 76.4 & 83.3 & 72.1\\
      \hline
      ESIR (2019)  & 93.3 & 90.2 & - & 91.3 & - & 76.9 & 79.6 & 83.3 & 78.1\\
      \hline
      MORAN (2019) & 91.2 & 88.3 & 95.0 & 92.4 & 91.7 & 68.8 & 76.1 & 77.4 & 71.2\\
      \hline
      Mask TextSpotter (2019) *\textdagger & \textbf{95.3} & \dunderline{0.7pt}{91.8} & 95.0 & \textbf{95.3} & \textbf{94.8} & 78.2 & 83.6 & \textbf{88.5} & 80.0\\
      \hline
      \hline
      \AlgoName (1 Block) & 92.9 & 89.2 & \dunderline{0.7pt}{96.5} & 93.8 & 93.2 & 81.8 & 84.5 & 85.1 & 82.7 \\
      \hline
      \AlgoName (2 Block)& 93.5 & 89.2 & 95.9 & \dunderline{0.7pt}{94.7} & 93.6 & 81.5 & 86.2 & 86.8 & 83.0\\
      \hline
      \AlgoName (3 Block) & \dunderline{0.7pt}{93.9} & 89.3 & 96.1 & 94.6 & 93.7 & \textbf{82.8} & 85.7 & 83.7 & 83.4\\
      \hline
      \AlgoName (4 Block) & 93.4 & 90.3 & \textbf{96.6} & 94.3 & 93.7 &  82.0 & \textbf{87.0} & 86.5 & \dunderline{0.7pt}{83.5}\\
      \hline
      \AlgoName (5 Block) & 93.6 & \textbf{92.7} & 96.3 & 93.9 & \dunderline{0.7pt}{94.0} &  \dunderline{0.7pt}{82.1} & \dunderline{0.7pt}{86.8} & \dunderline{0.7pt}{87.5} & \textbf{83.7}\\
      \hline
    \end{tabular}
  \end{center}
\egroup
\end{center}
\end{table*}
